disco: a toolkit for Distributional Control of Generative Models

Pre-trained language models and other generative models have revolutionized NLP and beyond. However, these models tend to reproduce undesirable biases present in their training data. Also, they may overlook patterns that are important but challenging to capture. To address these limitations, researchers have introduced distributional control techniques. These techniques, not limited to language, allow controlling the prevalence (i.e., expectations) of any features of interest in the model's outputs. Despite their potential, the widespread adoption of these techniques has been hindered by the difficulty in adapting complex, disconnected code. Here, we present disco, an open-source Python library that brings these techniques to the broader public.

==> scratchpad.tex <==




\section{Suggestions}

The previous experiments showcased the ease of use of the toolkit as well the power of the underlying theoretical framework. We can imagine many more applications: if we have a scorable feature on the samples from a generative model, we can control the generation.

\begin{itemize}
    \item having gold summaries, we could target some of their properties, a ROUGE score for example, in the outputs a seq2seq model;
    \item from the ``helpfulness score'' of a text, e.g. through a model learned from human feedback, we could align a generative CLM \textemdash similarly a Click Through Rate could be a signal to use if one is after attention;
    \item language models have been used to plan sequences of actions~\citep{} but we might want to impose preferences distributionally on the agent, if only to handle scarcity in the resources (tools, path, \dots);
    \item models can create great images but it's a politically loaded medium so, depending of the audience, we might want to make sure they are safe, and overall balanced;
    \item a very strong chess playing agent can be very boring if it always beats its human opponent, or always plays the same move.
\end{itemize}

